Reaping the Informational Surplus in Bayesian Persuasion

The Bayesian persuasion model studies communication between an informed sender and a receiver with a payoff-relevant action, emphasizing the ability of a sender to extract maximal surplus from his informational advantage. In this paper we study a setting with multiple senders, but in which the receiver interacts with only one sender of his choice: senders commit to signals and the receiver then chooses, at the interim stage, with which sender to interact. Our main result is that whenever senders are even slightly uncertain about each other's preferences, the receiver receives all the informational surplus in all equilibria of this game.

==> mixed.tex <==
% !TeX root = paper.tex

\section{Mixed Nash Equilibria}\label{sec:mixed}
In this section we extend the model to consider also mixed strategies by the senders.
Instead of each sender choosing a signal $\pi_i\in\Pi_i$, we now allow each sender $i$ to choose a distribution $\ppi_i$ over $\Pi_i$. Then, a signal
$\pi_i\sim\ppi_i$ is realized for each such sender, after which $R$ chooses one of the players, say $j$. The state is then realized, sender $j$ learns the state 
$\omega_{jR}\eqdef (\omega_j,\omega_R)$ and the receiver gets (only) the message $\pi_j(\omega_{jR})$ sent by the chosen player $j$. 
Finally, $R$ takes an action in $\A$ and payoffs of all players are realized.

We stress that in this game, the receiver chooses a sender with whom to interact {\em after} he observes the signal $\pi_i$ drawn from each sender $i$'s
distribution $\ppi_i$. Were he to make this choice after observing only the distributions $\ppi_i$, the model would be identical to one restricted to pure
strategies, since each $\ppi_i$ is equivalent to some $\pi_i$ in terms of the senders' and receiver's eventual utilities. The only role played by the {\em distribution}
$\ppi$ is in terms of possibly expanding the set of equilibria.

When defining pure Nash equilibria, we allowed the receiver some flexibility in his decision rule $D$. In this section, however, we will suppose that when there are multiple senders all of whose signals lead to the same, maximal expected utility for the receiver, he chooses one uniformly at random.
Thus, we fix the decision rule $D:\Pi_1\times\ldots\times\Pi_n\mapsto\Delta\left(\{1,\ldots,n\}\right)$ of the receiver as a uniformly-random choice of 
a sender $j$ from the set $\left\{j:\pi_j\succeq_R \pi_i ~\forall i\in\{1,\ldots,n\}\right\}$. 


\begin{definition}
A {\em Nash equilibrium (NE)} of the game is a profile  $\ppi=\left(\ppi_1,\ldots,\ppi_n\right)$ 
with the following property: There do not exist a sender $i$ and distribution $\ppi_i'$ over signals with
$$E\left[v_i(\pi_{D(\ppi_i',\ppi_{-i})})\right] > E\left[v_i(\pi_{D(\ppi)})\right],$$
where $(\ppi_i',\ppi_{-i})$ is the profile $\ppi$ but with $\ppi_i'$ replacing $\ppi_i$.
\end{definition}

As before, our main result is that in every NE of the game, the receiver only chooses fully-informative signals:
\begin{theorem}\label{thm:mixed}
	Let $\ppi$ be a NE of the game. Then with probability 1 the realized profile $\left(\pi_1,\ldots,\pi_n\right)$ satisfies the following:
	for every sender $j$  that is chosen by the receiver with positive probability it holds that $\pi_j$ is fully informative.
\end{theorem}


\begin{proofof}{Theorem~\ref{thm:mixed}}
Fix a NE $\ppi$, and suppose towards a contradiction that with positive probability, the realized profile $\left(\pi_1,\ldots,\pi_n\right)$ 
is such that a sender $j$ is chosen with positive probability, but that $\pi_j$ is not fully informative. Let $\eta>0$ denote
the probability that such a $\left(\pi_1,\ldots,\pi_n\right)$ is realized. This implies that, for every sender $i$,
the probability of realizing some $\pi_i$ that is not fully informative, under $\ppi_i$, is at least $\eta$.


We now develop some notation that will be helpful. Let $T_i = \supp\left(v_R(\ppi_i)\right)$ be the set of possible 
receiver payoffs attainable by a signal in sender $i$'s support, and denote by $\tau_i=\min T_i$.\footnote{Recall that the support of a random variable
is the smallest {\em closed} subset of values with measure 1, and so the minimum of $T_i$ exists.} 
Note that the receiver's utility from a fully-informative signal is maximal for him, and so must be weakly higher than all payoffs in $T_i$.
Furthermore, observe that if a signal is not fully-informative then the receiver's utility from following that signal's recommendations will be strictly lower
than his utility from following the recommendations of a fully-informative signal.

Let $N_{\min}=\left\{i: \tau_i\leq \tau_j~\forall~j\in\{1,\ldots,n\}\right\}$ be the set of senders $i$ with minimal $\tau_i$.
The following lemma states that all senders have the same minimal $\tau_i$.

In the proof, we use the following notation: First, we denote by $\ppi_{-i}$  the profile $\ppi$ with sender $i$ removed. Second,
we slightly misuse notation and write $D(\pi_{-i})$ as a uniformly-random choice of 
a sender $j$ from the set $\left\{j:\pi_j\succeq_R \pi_k ~\forall k\in\{1,\ldots,n\}\setminus\{i\}\right\}$.

\begin{lemma}\label{lem:equal-tau}
$\abs{N_{\min}}= n$.
\end{lemma}

\begin{proof}
Suppose not, and that $i\in N_{\min}$ and  $j\not\in N_{\min}$, for some senders $i\neq j$. Furthermore, suppose $j$ is the sender for whom $\tau_j$
is maximal: $\tau_j \geq \tau_k$ for all $k\in\{1,\ldots,n\}$.
Let $\zeta = P(\ppi_i = \pi_i\mid v_R(\pi_i)<\tau_j)$. Since $\tau_i\in\supp\left(v_R(\ppi_i)\right)$ and $\tau_i<\tau_j$, it must be the case
that $\zeta>0$.
Thus, under $\ppi_i$, with probability $\zeta>0$, sender $i$ chooses a signal that is never chosen by the receiver. Thus, conditional on him choosing
one of those signals, his utility will be $E\left[v_i(\pi_{D(\ppi_{-i})})\right]$.

We now construct a profitable deviation for sender $i$. Let $k$ and $\pi_k$ satisfy $v_i(\pi_k)\geq E\left[v_i(\pi_{D(\ppi_{-i})})\right]$.
Such a pair must exist: when players and signals are chosen randomly according to $D(\ppi_{-i})$, sender $i$'s expected utility is $E\left[v_i(\pi_{D(\ppi_{-i})})\right]$.
Thus, there must be some realization of $\pi_{D(\ppi_{-i})}$ that yields sender $i$ a weakly higher payoff.
Next, by Lemma~\ref{lem:i-improve}, there exists a signal $\pi_i'$ for sender $i$ that is strictly better than $\pi_k$ for both $i$ and the receiver. His profitable deviation is
$\ppi_i'$, which is the same as $\ppi_i$ except that the $\zeta$ measure of signals that are never chosen are replaced by $\pi_i'$.
\end{proof}

Henceforth, denote by $\tau=\tau_i$. Note that, since every sender plays a signal that is not fully informative with probability at least $\eta$,
the signals leading to receiver utility $\tau$ are not fully informative (since fully informative signals lead to utilities that are maximal 

Next, we will consider three cases:
\begin{itemize}
\item[(i)] $P(v_R(\ppi_i)=\tau)=0$ for all $i\in \{1,\ldots,n\}$.
\item[(ii)] $P(v_R(\ppi_i)=\tau)>0$ and $P(v_R(\ppi_j)=\tau)=0$ for some $i,j\in \{1,\ldots,n\}$.
\item[(iii)]  $P(v_R(\ppi_i)=\tau)>0$ for all $i\in \{1,\ldots,n\}$.
\end{itemize}


We begin with case (i). Let $i$ be any sender, and note that the equality $P(v_R(\ppi_i)=\tau)=0$ implies that for all $\eps>0$, 
$$P\left(v_R(\ppi_i)\in \left[\tau,\tau+\eps\right]\right)>0$$
(for otherwise, $\tau$ would not be in the support of $v_R(\ppi_i)$).
Thus, sender $i$ chooses a signal $\pi_i$ with $v_R(\pi_i)\in \left[\tau,\tau+\eps\right]$ with positive probability. Furthermore,
the probability that $i$'s signal is chosen by the receiver, when he plays such a signal, approaches 0 with $\eps$:
$$\lim_{\eps\rightarrow 0} P\left(D(\ppi)=i \mid v_R(\pi_i)\in \left[\tau,\tau+\eps\right]\right) = 0.$$

This is because, as $\eps$ approaches 0, the probability that there is some $j\neq i$ and $\pi_j$ such that $v_R(\pi_j)>\tau+\eps$ approaches 1, and
the receiver will choose the sender offering the signal with the highest $v_R$.

Now, $\ppi_i$ is $i$'s equilibrium strategy, which implies that $i$ is indifferent between all but a measure 0 of the signals in the support of $\ppi_i$.
That is, for each such signal, sender $i$ considers the expected utility from that signal: the probability that it is chosen by the receiver times the utility
 $i$ derives from it.
In equilibrium, the expected utility of a particular signal is equal for all signals. 
By the above, $i$ sometimes plays signals that are almost never chosen by the receiver, and this leads to utility arbitrarily close to
$E\left[v_i(\pi_{D(\ppi_{-i})})\right]$ for him. The equilibrium indifference then implies that this same expected utility is obtained by sender $i$
for all the signals in his support. Thus, his equilibrium payoff is arbitrarily close to $E\left[v_i(\pi_{D(\ppi_{-i})})\right]$.

We now construct a  profitable deviation for sender $i$, as follows. 
Let $j\neq i$ and $\pi_j$ satisfy $v_i(\pi_j)\geq v_i(\pi_k)$ for all senders $k\neq i$ and signals $\pi_k\in\supp(\ppi_k)$.
That is, $\pi_j$ is the best signal for sender $i$ played in equilibrium by any other sender $j$.
If $\pi_j$ is not fully-informative, then
by Lemma~\ref{lem:i-improve} there exists a signal $\pi_i'$ for sender $i$ that is strictly better than $\pi_j$ for both $i$ and the receiver. His profitable deviation is
to play $\pi_i'$ always, a deviation that contradicts the assumption that $\ppi$ is a NE.

If $\pi_j$ is fully informative, then there are two cases. First, if $v_i(\pi_j)>E\left[v_i(\pi_{D(\ppi_{-i})})\right]$, then sender $i$ has a profitable deviation to always play
a fully-informative signal. If $v_i(\pi_j)=E\left[v_i(\pi_{D(\ppi_{-i})})\right]$, then it must be the case that for all signals $\pi_k\in\supp(\ppi_k)$ the equality
 $v_i(\pi_k)=E\left[v_i(\pi_{D(\ppi_{-i})})\right]$ holds. If some such $\pi_k$ is not fully-informative, then sender $i$ can invoke the same profitable deviation as
 above, by simulating and improving upon $\pi_k$ as in Lemma~\ref{lem:i-improve}. 
 If, on the other hand, all such $\pi_k$'s are fully informative, then whenever the receiver chooses a signal from any sender other than $i$,
 that signal is fully informative. But this implies that the receiver always has a a fully-informative signal available, and, since such a signal is optimal for him,
 he will always choose it. This is a contradiction.
 

We now consider case (ii), that $P(v_R(\ppi_i)=\tau)>0$ and $P(v_R(\ppi_j)=\tau)=0$ for some $i,j\in \{1,\ldots,n\}$.
Here, observe that signals $\pi_i\in\supp(\ppi_i \mid v_R(\ppi_i)=\tau)$ are played by sender $i$ with positive probability, but are chosen with probability
0 (since any signal of sender $j$ will be preferred over $\pi_i$).  As above, this again implies that, by $i$'s indifference between all the signals in the support
of $\ppi_i$, sender
$i$'s equilibrium payoff is arbitrarily close to $E\left[v_i(\pi_{D(\ppi_{-i})})\right]$.

We can thus construct the same profitable deviation for sender $i$ as in case (i), by either replacing $\ppi$ by $\pi_i'$ that simulates  
$\pi_j$, where $\pi_j$ satisfies $v_i(\pi_j)\geq v_i(\pi_k)$ for all senders $k$ and signals $\pi_k\in\supp(\ppi_k)$, or by replacing $\ppi$ by a fully-informative
signal, if all such $\pi_j$'s are fully-informative.

Finally, we consider case (iii), that  $P(v_R(\ppi_i)=\tau)>0$ for all $i\in \{1,\ldots,n\}$. We will again construct a profitable deviation,
this time along the same lines as the one constructed in Theorem~\ref{thm:pure}.
Note that, under case (iii), $P\left(v_R\left(\pi_{D(\ppi)}\right)=\tau\right)>0$.

% Fix some sender $i$, and let $\ell$ and $\pi_\ell$ satisfy $v_i(\pi_\ell)\geq v_i(\pi_k)$ for all senders $k$ and signals $\pi_k\in\supp(\ppi_k)$. That is, $\pi_\ell$
% is the signal yielding highest utility to sender $i$ played by any other sender. We consider two cases. 

Again, we consider three cases. First, if for some sender $i$ it holds that $E[v_i(\ppi_i)\mid v_R(\pi_{D(\ppi)})=\tau] \geq E[v_i(\ppi_j)\mid v_R(\pi_{D(\ppi)})=\tau]$
for all $j\neq i$, with a strict inequality for at least one such $j$,
then sender $i$ has the following profitable deviation:
Instead of choosing $(\ppi_i\mid v_R(\ppi_i)=\tau)$, sender $i$ chooses $\ppi_i'$: Replace every $\pi_i\in\supp(\ppi_i\mid v_R(\ppi_i)=\tau)$ with $\pi_i'$ such that with (arbitrarily) small probability $\eps$ signal $\pi_i'$ is realized as a fully-informative signal---that is, it is realized as $\arg\max_{a\in\A} u_R(a,\omega_R)$ in every state $\omega_R\in\Omega_R$---and with probability $1-\eps$ it is realized as $\pi_i$. 
	For any $\eps>0$, the new signal distribution $\ppi_i'$ will be more informative than $\ppi_j$, and so the receiver will choose sender $i$ with probability 1 (conditional on $v_R(\pi_{D(\ppi)})=\tau$), leading to a strict increase in $i$'s utility.
	Since $\eps$ can be arbitrarily small, this does not harm sender $i$ much, and so for small enough $\eps$ the overall gain from the deviation is positive.

The second case is if for some sender $i$ it holds that $E[v_i(\ppi_i)\mid v_R(\pi_{D(\ppi)})=\tau] < E[v_i(\ppi_j)\mid v_R(\pi_{D(\ppi)})=\tau]$ for
some $j\neq i$.
In this case, sender $i$ has the following profitable deviation: Replace $(\ppi_i\mid v_R(\ppi_i)=\tau)$ by $\ppi_i'$, where $\ppi_i'$ is the ``simulation''
of  $(\ppi_j\mid v_R(\ppi_j)=\tau)$. That is,  for each $\pi_j\in\supp(\ppi_j\mid v_R(\ppi_j)=\tau)$,
$i$ plays the simulation $\pi_i'$ of $\pi_j$ guaranteed to exist by Lemma~\ref{lem:simulate}. Under this deviation, sender $i$'s
utility, conditional on receiver utility equal to $\tau$, is equal to $E[v_i(\ppi_j)\mid v_R(\pi_{D(\ppi)})=\tau]$. By assumption, this is a
strict improvement over $E[v_i(\ppi_i)\mid v_R(\pi_{D(\ppi)})=\tau]$.

The third case is if for some sender $i$ it holds that
$E[v_i(\ppi_i)\mid v_R(\pi_{D(\ppi)})=\tau] = E[v_i(\ppi_j)\mid v_R(\pi_{D(\ppi)})=\tau]$
for all $j\neq i$. Note that this expected utility is thus equal to $E[v_i(\pi_{D(\ppi)})\mid v_R(\pi_{D(\ppi)})=\tau]$.
Let $\ell$ and $\pi_\ell$ satisfy $v_i(\pi_\ell)\geq v_i(\pi_k)$ for all senders $k\neq i$ and signals $\pi_k\in\supp(\ppi_k)$. That is, $\pi_\ell$
 is the signal yielding highest utility to sender $i$ played by any other sender.
In this third case, as in case (i) above, sender $i$ has the following profitable deviation:  
If $\pi_\ell$ is not fully-informative, replace $(\ppi_i\mid v_R(\ppi_i)=\tau)$ by $\pi_i'$, where $\pi_i'$ is the improvement on the simulation of $\pi_\ell$ guaranteed to exist by Lemma~\ref{lem:i-improve}. 
By the lemma and assumption, $v_i(\pi_i')>v_i(\pi_\ell)\geq E[v_i(\ppi_i)\mid v_R(\pi_{D(\ppi)})=\tau]$.
Since sender $i$ deviates to a signal that yields him the highest possible utility over all other senders' signals, this deviation is profitable.

If $\pi_\ell$ is fully informative and $v_i(\pi_\ell)> E[v_i(\ppi_i)\mid v_R(\pi_{D(\ppi)})=\tau]$, replace $(\ppi_i\mid v_R(\ppi_i)=\tau)$ by a fully-informative signal.
This again is a profitable deviation. 

Finally, suppose $\pi_\ell$ is fully informative and $v_i(\pi_\ell)= E[v_i(\ppi_i)\mid v_R(\pi_{D(\ppi)})=\tau]=E[v_i(\pi_{D(\ppi)})\mid v_R(\pi_{D(\ppi)})=\tau]$.
 The equality $v_i(\pi_\ell)=E[v_i(\pi_{D(\ppi)})\mid v_R(\pi_{D(\ppi)})=\tau]$ implies that for all senders $k\neq i$ and signals $\pi_k\in\supp\left(\ppi_k \mid v_R(\ppi_k)=\tau\right)$ the equality
 $v_i(\pi_k)=E[v_i(\pi_{D(\ppi)})\mid v_R(\pi_{D(\ppi)})=\tau]$ holds. If some such $\pi_k$ is not fully-informative, then sender $i$ can invoke the same profitable deviation as
 above, by simulating and improving upon $\pi_k$ as in Lemma~\ref{lem:i-improve}. 
 If, on the other hand, all such $\pi_k$'s are fully informative, then whenever the receiver chooses a signal $\pi_k$ from any sender other than $i$, and obtains utility
 $v_R(\pi_k)=\tau$, that signal is fully informative. However, this is a contradiction, since $\tau$ is strictly less than the receiver's optimal utility.
\end{proofof}








==> outline.tex <==
% !TeX root = paper.tex

\subsection{Outline}
The next section contains a review of the related literature. This is followed by Section \ref{sec:model}, in which
we describe the basic model of the game and the underlying assumptions. 

In Section~\ref{sec:equilibrium} we present the main result of the paper: In every pure equilibrium, a sender that is chosen by the receiver with positive probability in the interim stage chooses a signal that divulges all payoff-relevant information to the receiver. This is followed by
Section~\ref{sec:mixed}, which proves the same result for mixed equilibria. Finally, Section~\ref{sec:conc} concludes.
